FinRL: Deep Reinforcement Learning Framework to Automate Trading in Quantitative Finance

Deep reinforcement learning (DRL) has been envisioned to have a competitive edge in quantitative finance. However, there is a steep development curve for quantitative traders to obtain an agent that automatically positions to win in the market, namely \textit{to decide where to trade, at what price} and \textit{what quantity}, due to the error-prone programming and arduous debugging. In this paper, we present the first open-source framework \textit{FinRL} as a full pipeline to help quantitative traders overcome the steep learning curve. FinRL is featured with simplicity, applicability and extensibility under the key principles, \textit{full-stack framework, customization, reproducibility} and \textit{hands-on tutoring}. Embodied as a three-layer architecture with modular structures, FinRL implements fine-tuned state-of-the-art DRL algorithms and common reward functions, while alleviating the debugging workloads. Thus, we help users pipeline the strategy design at a high turnover rate. At multiple levels of time granularity, FinRL simulates various markets as training environments using historical data and live trading APIs. Being highly extensible, FinRL reserves a set of user-import interfaces and incorporates trading constraints such as market friction, market liquidity and investor's risk-aversion. Moreover, serving as practitioners' stepping stones, typical trading tasks are provided as step-by-step tutorials, e.g., stock trading, portfolio allocation, cryptocurrency trading, etc.

==> NeurIPS_2020_version/Section1_Introduction.tex <==
\section{Introduction}

Deep reinforcement learning (DRL), which balances exploration (of uncharted territory) and exploitation (of current knowledge), has been recognized as an advantageous approach for automated stock trading. DRL framework is powerful in solving dynamic decision making problems by learning through interaction with an unknown environment, and thus providing two major advantages - portfolio scalability and market model independence \cite{buehler2019deep}. In quantitative finance, stock trading is essentially making dynamic decisions, namely \textit{to decide where to trade, at what price, and what quantity}, over a highly stochastic and complex stock market. As a result, DRL provides useful toolkits for stock trading \cite{hull2009options,xiong2018practical,zhang2020deep,yang2020,Dang2019ReinforcementLI,DRL_automate,li_a2c_2018}. Taking many complex financial factors into account, DRL trading agents build a multi-factor model and provide algorithmic trading strategies, which are difficult for human traders \cite{bekiros2010fuzzy,zhang2017online,kim2017intelligent,Jiang2017ADR}.

Preceding DRL, conventional reinforcement learning (RL) \cite{sutton2018reinforcement} has been applied to complex financial problems \cite{luenberger1997investment}, including option pricing, portfolio optimization and risk management. Moody and Saffell \cite{moody2001learning} utilized policy search and direct RL for stock trading. Deng \textit{et al.} \cite{Deng2017DeepDR} showed that applying deep neural networks profits more. There are industry practitioners who have explored trading strategies fueled by DRL, since deep neural networks are significantly powerful at approximating the expected return at a state with a certain action. With the development of more robust models and strategies, general machine learning approaches and DRL methods in specific are becoming more reliable. For example, DRL has been implemented on sentimental analysis on portfolio allocation \cite{li2019optimistic,Jiang2017ADR} and liquidation strategy analysis \cite{bao2019multi}, showing the potential of DRL on various financial tasks.

However, to implement a DRL or RL driven trading strategy is nowhere near as easy. The development and debugging processes are arduous and error-prone. Training environments, managing intermediate trading states, organizing training-related data and standardizing outputs for evaluation metrics - these steps are standard in implementation yet time-consuming especially for beginners. Therefore, we come up with a beginner-friendly library with fine-tuned standard DRL algorithms. It has been developed under three primary principles:
\begin{itemize}
  \item \textbf{Completeness}. Our library shall cover components of the DRL framework completely, which is a fundamental requirement;
  \item \textbf{Hands-on tutorials}. We aim for a library that is friendly to beginners. Tutorials with detailed walk-through will help users to explore the functionalities of our library;
  \item \textbf{Reproducibility}. Our library shall guarantee reproducibility to ensure the transparency and also provide users with confidence in what they have done.
\end{itemize}
%This spawns a unified and complete library where developers are able to efficiently explore ideas through high-level model operations, and customize their own environment modules when necessary.

In this paper, we present a three-layered \textit{FinRL} library that streamlines the development stock trading strategies. FinRL provides common building blocks that allow strategy builders to configure stock market datasets as virtual environments, to train deep neural networks as trading agents, to analyze trading performance via extensive backtesting, and to incorporate important market frictions. On the lowest level is environment, which simulates the financial market environment using actual historical data from six major indices with various environment attributes such as closing price, shares, trading volume, technical indicators etc. In the middle is the agent layer that provides fine-tuned standard DRL algorithms (DQN \cite{lillicrap2015continuous}\cite{mnih2015human}, DDPG \cite{lillicrap2015continuous}, Adaptive DDPG \cite{li2019optimistic}, Multi-Agent DDPG \cite{lowe2017multi}, PPO \cite{schulman2017proximal}, SAC \cite{haarnoja2018soft}, A2C \cite{mnih2016asynchronous} and TD3 \cite{Dankwa2019TwinDelayedDA}, etc.), commonly used reward functions and standard evaluation baselines to alleviate the debugging workloads and promote the reproducibility. The agent interacts with the environment through properly defined reward functions on the state space and action space. The top layer includes applications in automated stock trading, where we demonstrate three use cases, namely single stock trading, multiple stock trading and portfolio allocation. 

The contributions of this paper are summarized as follows:
\begin{itemize}
  \item FinRL is an open source library specifically designed and implemented for quantitative finance. Trading environments incorporating market frictions are used and provided.   
  %designed specifically for automated stock trading
  %\item Customization of trading time steps is feasible.
  \item Trading tasks accompanied by hands-on tutorials with built-in DRL agents are available in a beginner-friendly and reproducible fashion using Jupyter notebook. Customization of trading time steps is feasible.
  \item FinRL has good scalability, with a broad range of fine-tuned state-of-the-art DRL algorithms. Adjusting the implementations to the rapid changing stock market is well supported.
  \item Typical use cases are selected and used to establish a benchmark for the quantitative finance community. Standard backtesting and evaluation metrics are also provided for easy and effective performance evaluation. 
\end{itemize}

The remainder of this paper is organized as follows. Section 2 reviews related works. Section 3 presents FinRL Library. Section 4 provides evaluation support for analyzing stock trading performance. We conclude our work in Section 5. 


==> NeurIPS_2020_version/Section2_ExistingWorks.tex <==
\section{Related Works}

We review related works on relevant open source libraries and existing applications of DRL in finance.  

\subsection{State-of-the-Art Algorithms}

Recent works can be categorized into three approaches: value based algorithm, policy based algorithm, and actor-critic based algorithm. FinRL has consolidated and elaborated upon those algorithms to build financial DRL models. There are a number of machine learning libraries that share similar features as our FinRL library. \
%In Table 1 we compare with them from different perspectives.

%\begin{table*}[htb]
%\caption{Comparison of RL Libraries}
%\begin{tabular}{|l|l|l|l|l|}
%\hline
%\textbf{Libraries}       & \textbf{SOTA RL}        & %\textbf{Doc.}           & \textbf{Pip Installer}        & \textbf{Finance Customization}       \\ \hline
%\textbf{FinRL}       & Yes     & Yes     & Yes     & Yes     %    \\ \hline
%\textbf{OpenAI Gym}       & Yes     & No     & Yes     & No  %       \\ \hline
%\textbf{Google Dopamine}         & Yes     & Yes     & Yes   %  & No         \\ \hline
%\textbf{RLlib}          & Yes     & Yes     & Yes     & No   %      \\ \hline
%\textbf{RLlab}             & Yes     & Yes     & Yes     & No %        \\ \hline
%\textbf{Personae}         & Yes     & No     & Yes     & No  %       \\ \hline
%\textbf{Tensorforce}        & Yes     & Yes     & Yes     & No         \\ \hline
%\textbf{Horizon}        & Yes     & No     & No     & No         \\ \hline
%\end{tabular}
%\end{table*}


\begin{itemize}
\item \textbf{OpenAI Gym} \cite{brockman2016openai} is a popular open source library that provides a standardized set of task environments. OpenAI Baselines \cite{baselines} implements high quality deep reinforcement learning algorithms using gym environments. Stable Baselines \cite{stable-baselines} is a fork of OpenAI Baselines with code cleanup and user-friendly examples.

\item \textbf{Google Dopamine} \cite{castro18dopamine} is a research framework for fast prototyping of reinforcement learning algorithms. It features plugability and reusability. 

\item \textbf{RLlib} \cite{liang2018rllib} provides high scalability with reinforcement learning algorithms. It has modular framework and is very well maintained.

%\item \textbf{TensorLayer} \cite{dong2017tensorlayer} is a deep learning library with RL support, designed for researchers and engineers to customize neural networks for real-world applications. TensorLayer is a wrapper of TensorFlow and uses the OpenAI Gym module as environment, not user-friendly for financial tasks.

%\item \textbf{RLlab} \cite{duan2016benchmarking} is a reinforcement learning framework for developing continuous control tasks. 

%\item \textbf{Personae} \cite{Personae} includes DRL algorithms and applies them to financial tasks. It includes a basic environment simulating financial market supporting stock and future. However, it lacks market frictions, nor does it allow customization. 

%\item \textbf{Tensorforce} \cite{lift-tensorforce} Tensorforce is an extension to Tensorflow and gains all benefits of using Tensorflow. However, the code is complicated which makes it not easy for beginners to get hands on.

\item \textbf{Horizon} \cite{gauci2018horizon}  is a DL-focused framework dominated by PyTorch, whose main use case is to train RL models in the batch setting.
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{DRL in Finance}

Recent works show that DRL has many applications in quantitative finance \cite{RL_survey}.

Stock trading is usually considered as one of the most challenging applications due to its noisy and volatile features. Many researchers have explored various approaches using DRL \cite{nechchi2016reinforcement, Nan2020SentimentAK, Dang2019ReinforcementLI, Corazza2014QLearningBasedFT, zhang2020deep, Ganesh2018DeepRL}. Volatility scaling can be incorporated with DRL to trade futures contracts \cite{zhang2020deep}. By adding a market volatility term to reward functions, we can scale up the trade shares with low volatility, and vice versa. News headline sentiments and knowledge graphs can also be combined with the time series stock data to train an optimal policy using DRL \cite{Nan2020SentimentAK}. High frequency trading with DRL is also a hot topic \cite{Ganesh2018DeepRL}. Deep Hedging \cite{buehler2019deep, Cao2019DeepHO} represents hedging strategies with neural networks learned by modern DRL policy search. This application has shown two key advantages of the DRL approach in quantitative finance, which are scalability and model independent. It uses DRL to manage the risk of liquid derivatives, which indicates further extension of our library into other asset classes and topics. 

%Cryptocurrency is considered as a significant and rising element in today's digital financial market. Crypto markets led by Bitcoin (BTC)  \cite{Sapuric2014BitcoinIV} are considered as more volatile than stock market. We can also apply DRL to those markets performing automated trading \cite{Lucarelli2019ADR}, portfolio allocation \cite{Jiang2017CryptocurrencyPM}, and market making \cite{Sadighian2019DeepRL}.

==> NeurIPS_2020_version/Section3_Architecture.tex <==
\section{The Proposed FinRL Library}

FinRL library consists of three layers: environments, agents and applications. We first describe the overall architecture, and then present each layer.
%the simulated trading environment layer and DRL trading agent layer, respectively.

\subsection{Architecture of the FinRL Library}

The architecture of the FinRL library is shown in Fig. \ref{overview}, and its features are summarized as follows:
\begin{itemize}
    \item \textbf{Three-layer architecture}: The three layers of FinRL library are stock market environment, DRL trading agent, and stock trading applications. The agent layer interacts with the environment layer in an exploration-exploitation manner, whether to repeat prior working-well decisions or to make new actions hoping to get greater rewards. The lower layer provides APIs for the upper layer, making the lower layer transparent to the upper layer.
    \item \textbf{Modularity}: Each layer includes several modules and each module defines a separate function. One can select certain modules from any layer to implement his/her stock trading task. Furthermore, updating existing modules is possible.
    \item \textbf{Simplicity, Applicability and Extendibility}: Specifically designed for automated stock trading, FinRL presents DRL algorithms as modules. In this way, FinRL is made accessible yet not demanding. FinRL provides three trading tasks as use cases that can be easily reproduced. Each layer includes reserved interfaces that allow users to develop new modules. 
    \item \textbf{Better Market Environment Modeling}: We build a trading simulator that replicates live stock market and provides backtesting support that incorporates important market frictions such as transaction cost, market liquidity and the investor's degree of risk-aversion. All of those are crucial among key determinants of net returns. 
\end{itemize}

%Each layer of FinRL library is described as follows.

%On the environment layer, six frequently-referred-to index, NASDAQ-100, DJIA, S\&P 500, SSE 50, CSI 300, HSI are included. 

%On the agent layer, FinRL provides both RL and DRL fine-tuned algorithms, which can be directly used for and tested in user's stock trading tasks. Conventional learning algorithms include value iteration and policy iteration, which provide validations on small data sets for developing DRL algorithms. DRL agents include DQN \cite{mnih2015human}, DDPG \cite{lillicrap2015continuous}, Adaptive DDPG \cite{li2019optimistic}, Multi-Agent DDPG \cite{lowe2017multi}, PPO \cite{schulman2017proximal}, SAC \cite{haarnoja2018soft}, A2C \cite{mnih2016asynchronous} and TD3 \cite{fujimoto2018addressing} algorithms. 

%On the application layer, FinRL provides application demonstrations and benchmark tests. Benchmark tests include both conventional RL \& DRL algorithms that are trained with tens of stocks. The benchmark tests serve as preliminary verification for users when they develop their own strategies. The application demonstrations include single stock trading using DQN and DDPG, portfolio allocation using Adaptive DDPG, and liquidation strategy analysis using MADDPG.

%\begin{figure}[t]
%\centering
%\includegraphics[height=3.5cm]{image/state521.png}
%\caption{State transition diagram.}
%\label{fig2}
%\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[height=7.0cm]{image/frame530.png}
\caption{An overview of our FinRL library. It consists of three layers: application layer, DRL agent layer, and the finance market environment layer.}
\label{overview}
\end{figure*}


==> NeurIPS_2020_version/Section3_Environment.tex <==
\subsection{Environment: Time-driven Trading Simulator}

Considering the stochastic and interactive nature of the automated stock trading tasks, a financial task is modeled as a Markov Decision Process (MDP) problem. The training process involves observing stock price change, taking an action and reward's calculation to have the agent adjusting its strategy accordingly. By interacting with the environment, the trading agent will derive a trading strategy with the maximized rewards as time proceeds.

%introduction
Our trading environments, based on OpenAI Gym framework, simulate live stock markets with real market data according to the principle of time-driven simulation \cite{brockman2016openai}. FinRL library strives to provide trading environments constructed by six datasets across five stock exchanges. 
%The state space representing the environment is used to pick the action in the action state and the reward as incentive. Every trading day, price of stocks in the state space changes and the agent takes trading actions on this basis.  

%It serves with supervision under real market and is more realistic and robust compared to artificial environment for DRL.
%why real market
%data set 

\subsubsection{State Space, Action Space, and Reward Function} We give definitions of the state space, action space and reward function.

\textbf{State space $\mathcal{S}$}.
The state space describes the observations that the agent receives from the environment. Just as a human trader needs to analyze various information before executing a trade, so our trading agent observes many different features to better learn in an interactive environment. We provide various features for users:
\begin{itemize}
\item Balance ${b}_{t}\in \mathbb{R}_+$: the amount of money left in the account at the current time step $t$.
\item Shares own $\bm{h}_{t}\in \mathbb{Z}_+^{n}$: current shares for each stock, $n$ represents the number of stocks.
\item Closing price $\bm{p}_{t}\in \mathbb{R}_+^{n}$: one of the most commonly used feature.
\item Opening/high/low prices $\bm{o}_{t}, \bm{h}_{t}, \bm{l}_{t}\in \mathbb{R}_+^{n}$: used to track stock price changes.
\item Trading volume $\bm{v}_{t}\in \mathbb{R}_+^{n}$: total quantity of shares traded during a trading slot.
\item Technical indicators: Moving Average Convergence Divergence (MACD) $\bm{M}_t \in \mathbb{R}^{n}$ and Relative Strength Index (RSI) $\bm{R}_t \in \mathbb{R}_+^{n}$, etc.
\item Multiple-level of granularity: we allow data frequency of the above features to be daily, hourly or on a minute basis.
\end{itemize}

\textbf{Action space $\mathcal{A}$}. 
The action space describes the allowed actions that the agent interacts with the environment. Normally, $a \in \mathcal{A}$ includes three actions: $a \in \{-1, 0, 1\}$,  where $-1, 0, 1$ represent selling, holding, and buying one stock. Also, an action can be carried upon multiple shares. We use an action space $\{-k,...,-1, 0, 1, ..., k\}$, where $k$ denotes the number of shares. For example, "Buy 10 shares of AAPL" or "Sell 10 shares of AAPL" are $10$ or $-10$, respectively.
%A continuous action space needs to be normalized to $[-1, 1]$, since the policy is defined on a Gaussian distribution, which needs to be normalized and symmetric.

%The reward function $r(s,a,s')$

\textbf{Reward function $r(s, a, s')$} is the incentive mechanism for an agent to learn a better action. There are many forms of reward functions. We provide commonly used ones \cite{RL_survey} as follows:
\begin{itemize}
\item The change of the portfolio value when action $a$ is taken at state $s$ and arriving at new state $s'$ \cite{Deng2017DeepDR, xiong2018practical,Dang2019ReinforcementLI,Nan2020SentimentAK, yang2020}, i.e., $r(s,a,s') =  v' - v$,
where $v'$ and $v$ represent the portfolio values at state $s'$ and $s$, respectively.
\item The portfolio log return when action $a$ is taken at state $s$ and arriving at new state $s'$ \cite{huang2018financial}, i.e., $r(s,a,s') =  \log(\frac{v'}{v})$.
\item The Sharpe ratio for periods $t=\{1,...,T\}$ \cite{jin2016portfolio, Moody1998PerformanceFA}, i.e., $S_T = \frac{\text{mean}(R_t)}{\text{std}(R_t)}$, where $ R_t =  v_t - v_{t-1}$. 

\item FinRL also supports user defined reward functions to include risk factor or transaction cost term such as in \cite{Deng2017DeepDR,zhang2020deep,buehler2019deep}
\end{itemize} 

%\textbf{Action-value function $Q_{\pi}(s, a)$}.
%Action-value function $Q_{\pi}(s, a)$ means the expected value of taking action $a$ in state $s$ under policy $\pi$.
\subsubsection{Standard and User Import Datasets}

The application of DRL in finance is different from that in other fields, such as playing chess and card games \cite{silver2016mastering,Zha2019ExperienceRO}; the latter inherently have clearly defined rules for environments. 
Various finance markets require different DRL algorithms to get the most appropriate automated trading agent. 
Realizing that setting up training environment is a time-consuming and laborious work, FinRL provides six environments based on representative listings, including NASDAQ-100, DJIA, S\&P 500, SSE 50, CSI 300, and HSI, plus one user-defined environment. With those efforts, this library frees users from tedious and time-consuming data pre-processing workload.

We are well aware that users may want to train trading agents on their own data sets. FinRL library provides convenient support to user imported data to adjust the granularity of time steps. We specify the format of the data for each of the use cases. Users only need to pre-process their data sets according to our data format instructions. 
%Stock statistics and indicators can be calculated using stock price data, which provides users more features for the construction of the state space. For example, MACD and RSI are calculated based on historical stock close prices. Furthermore, indicators such as period total return and Sharpe ratio can be used to assist users in performance evaluation.

%\textbf{NASDAQ-100 index constituents}: Its 100 constituents are characterized by high %technology, high growth and non-financial. Training in such an environment gets agent to %capture the financial trends of technology.
%
%\textbf{Dow Jones Industrial Average (DJIA) index constituents}: DJIA is the most cited %market indicator for overall market performance. It is made up of 30 constituents that %best represent their industries respectively. %Many researches select DJIA as an %indicator of overall market performance for their agents.
%
%\textbf{Standard \& Poor's 500 (S\&P 500) index constituents}: The S\&P 500 index %consists of 500 largest U.S. publicly traded companies.
%
%\textbf{HSI Index constituents:} Hang Seng Index (HSI) is the most widely quoted %indicator of the performance of the Hong Kong stock market. HSI constituent securities %are grouped into Finance, Utilities, Properties and Commerce \& Industry \cite{HSI}. 
%
%\textbf{SSE 50 Index constituents:} SSE 180 Index includes constituents with best %representation of A shares listed at Shanghai Stock Exchange (SSE) with considerable %size and liquidity. Listed companies are classified into 10 industries \cite{SSE}. 
%
%\textbf{CSI 300 Index constituents:} CSI 300 Index consists of the 300 largest and most %liquid A-share stocks listed on Shenzhen Stock Exchange or on SSE; the performance of %constituents very much reflect the overall performance of China A-share market %\cite{CSI300}.

%\subsubsection{User Import Data}

% User-defined Environment

\subsection{Deep Reinforcement Learning Agents}

\begin{figure*}[t]
\centering
\includegraphics[width=1.15\textwidth]{image/compare_4.PNG}
\caption{Comparison of DRL algorithms.}
\label{compare}
\end{figure*}

FinRL library includes fine-tuned standard DRL algorithms, namely, DQN \cite{lillicrap2015continuous}\cite{mnih2015human}, DDPG \cite{lillicrap2015continuous}, Multi-Agent DDPG \cite{lowe2017multi}, PPO \cite{schulman2017proximal}, SAC \cite{haarnoja2018soft}, A2C \cite{mnih2016asynchronous} and TD3 \cite{Dankwa2019TwinDelayedDA}. We also allow users to design their own DRL algorithms by adapting these DRL algorithms, e.g., Adaptive DDPG \cite{li2019optimistic}, or employing ensemble methods \cite{yang2020}. The comparison of DRL algorithms is shown in Fig. \ref{compare}

The implementation of the DRL algorithms are based on OpenAI Baselines \cite{baselines} and Stable Baselines \cite{stable-baselines}.


==> NeurIPS_2020_version/Section4_Evaluation.tex <==
\section{Evaluation of Trading Performance}

Standard metrics and baseline trading strategies are provided to support trading performance analysis. FinRL library follows a training-validation-testing flow to design a trading strategy. 
%FinRL also considers many trading constraints to perform backtesting tests.

\subsection{Standard Performance Metrics}
FinRL provides five evaluation metrics to help users evaluate the stock trading performance directly, which are final portfolio value, annualized return, annualized standard deviation, maximum drawdown ratio, and Sharpe ratio.

%\textbf{Final portfolio value}: portfolio value at the end of the trading stage.
%
%\textbf{Annualized return}: geometric average amount of money earned by the agent each %year over the time period. 
%
%\textbf{Annualized standard deviation}: annualized standard deviation of the portfolio %return $R_{p}$.
%
%\textbf{Maximum drawdown ratio}: the maximum percentage loss during the trading eriod.
%% FinRL pushes back at any historical point in the selected cycle, then find the nadir %of total assets. 
%
%\textbf{Sharpe ratio:} the average return earned in excess of the risk-free rate per %unit of volatility or total risk:
%\begin{equation}
%\text{Sharpe Ratio} =\frac{\mathbb{E}\left(R_{p}\right)-R_{f}}{\sigma_{p}},
%\end{equation}
%where $\mathbb{E}\left(R_{p}\right)$ is expected return rate, $R_{f}$ is risk-free %rate, and $\sigma_{p}$ is the standard deviation of $R_{p}$. 
 
\subsection{Baseline Trading Strategies}
Baseline trading strategies should be well-chosen and follow industrial standards. The strategies will be universal to measure, standard to compare with, and easy to implement. In FinRL library, traditional trading strategies serve as the baseline for comparing with DRL strategies. Investors usually have two objectives for their decisions: the highest possible profits and the lowest possible risks of uncertainty \cite{sharpe1970portfolio}. FinRL uses five conventional strategies, namely passive buy-and-hold trading strategy \cite{Malkiel2003PassiveIS}, mean-variance strategy \cite{meanvariance2012}, and min-variance strategy \cite{meanvariance2012}, momentum trading strategy \cite{Foltice2015ProfitableMT}, and equal-weighted strategy to address these two mutually limiting objectives and the industrial standards.

%\textbf{Passive Trading Strategy} \cite{Malkiel2003PassiveIS}: is a popular, very easy to implement, and lucrative strategy among investors. With minimal trading activities, investors simply buy and hold index ETFs \cite{Tarassov2016ExchangeTF} to replicate a broad market index or indices. Popular index ETFs are: SPDR S\&P 500 ETF Trust (SPY) and Vanguard 500 Index Fund (VOO) for S\&P 500 Index, SPDR Dow Jones Industrial Average ETF Trust (DIA) for Dow Jones Industrial Average, Invesco QQQ Trust Series 1 (QQQ) for Nasdaq 100 index, etc.

%\textbf{Mean-Variance Strategy} \cite{meanvariance2012}: to achieve an optimal balance between the risks and profits, or the highest Sharpe ratio. The objective of the mean-variance strategy is to minimize risk for a given level of expected return:
%\begin{equation}
%\begin{split}
%&\underset{{w_i}}{\min}~\text{var}(r_p) \\
%&\text{subject~to}~\mathbb{E}(r_p) = \mu^*,~~ \sum w_i = 1,
%
%\end{split}
%\end{equation} where $r_p$ is the portfolio return, $w_i$ is the portfolio weights, and %$\mu^*$ is the expected or target return.

%\textbf{Min-Variance Strategy} \cite{meanvariance2012}: to find the portfolio with the smallest variance. It indicates a well-diversified portfolio that consists of individually risky assets, which are hedged when traded together, resulting in the lowest possible risk for the rate of expected return. The objective function of min-variance model is similar to mean-variance model without setting the target return.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training-Validation-Testing Flow}

\begin{figure}[t]
\centering
\includegraphics[scale=0.47]{image/data_4.PNG}
\caption{Data splitting.}
\label{data}
\end{figure}


%\begin{figure}[t]
%\centering
%\includegraphics[height=4.5cm]{image/MADDPG515.png}
%\caption{The liquidation process with independent, competitive and cooperative agents using the FinRL library.}
%\label{fig5}
%\vspace{-0.17in}
%\end{figure}

%\begin{figure*}[t]
%\centering
%\includegraphics[height=2.0cm]{image/timeline507.png}
%\caption{Data splitting.}
%\label{fig4}
%\end{figure*}



%\yanglet{To Bruce: need to give reasons about why this flow is necessary for financial tasks?}
With our use cases as instances, the stock market data are divided into three phases in Fig. \ref{data}. Training dataset is the sample of data to fit the DRL model. The model sees and learns from the training dataset. Validation dataset is used for parameter tuning and to avoid overfitting. Testing (trading) dataset is the sample of data to provide an unbiased evaluation of a fine-tuned model. Rolling window is usually associated with the training-validation-testing flow in stock trading because investors and portfolio managers may need to rebalance the portfolio and retrain the model periodically. FinRL provides flexible rolling window selection such as on a daily basis, monthly, quarterly, yearly or by user specified.

%Specifically, with our use cases as instances, the stock market data are divided into three phases in Figure \ref{data}.
%According to the standard workflow in quantitative finance, 

%\textbf{Training phase}: we use data from 01/01/2009 to 09/30/2015 to train the automated trading agents.

%\textbf{Validation phase}: we use data from 10/01/2015 to 12/31/2015 to validate the results and adjust key parameters, such as time slice's size and learning rate.

%\textbf{Testing/Trading phase}: we use data from 01/01/2016 to 05/08/2020 (unseen data) to evaluate the performance of the applications.


%In performance evaluation of RL algorithms, the portfolio value and stock index yield are compared in the form of curve graphs in fig.3), users can see the performance of the algorithm on the DJIA constituents' data. Then specific indicators are shown in Table 1, showing the risks of trading using algorithms.

%From the results of RL, we can conclude that DRL method have better performance on DJIA than traditional investment methods and RL methods. There are also differences among different DRL methods. The evaluation model of FinRL is multi-angled and effective.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Backtesting with Trading Constraints}

In order to better simulate practical trading, we incorporate trading constraints, risk-aversion and automated backtesting tools.

\textbf{Automated Backtesting}.
Backtesting plays a key role in performance evaluation. Automated backtesting tool is preferable because it reduces the human error. In FinRL library, we use the Quantopian pyfolio package \cite{pyfolio} to backtest our trading strategies. This package is easy to use and consists of various individual plots that provide a comprehensive image of the performance of a trading strategy. 

\textbf{Incorporating Trading Constraints}.
Transaction costs incur when executing a trade. There are many types of transaction costs, such as broker commissions and SEC fee. We allow users to treat transaction costs as a parameter in our environments:
\begin{itemize}
    \item Flat fee: a fixed dollar amount per trade regardless of how many shares traded.
    \item Per share percentage: a per share rate for every share traded, for example, 1/1000 or 2/1000 are the most commonly used transaction cost rate for each trade.
\end{itemize}
Moreover, we need to consider market liquidity for stock trading, such as bid-ask spread. Bid-ask spread is the difference between the prices quoted for an immediate selling action and an immediate buying action for stocks. In our environments, we can add the bid-ask spread as a parameter to the stock closing price to simulate real world trading experience. 
%Lastly, in order to address the risk-aversion of various traders, one may add the standard deviation of the portfolio returns into our reward function or simply use the risk-adjusted Sharpe ratio as the reward function.


\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{image/perform_1_3.png}
\caption{Performance of single stock trading using PPO in the FinRL library.}
\label{single_stock}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{image/perform_2_3.png}
\caption{Performance of multiple stock trading and portfolio allocation using the FinRL library.}
\label{fig3}
\end{figure*}

\begin{table*}[t]
		\centering
		\resizebox{\textwidth}{!}{
		\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}\hline
			2019/01/01-2020/09/23 & SPY  & QQQ&GOOGL & AMZN & AAPL  &  MSFT  &  S\&P 500 \\
			\hline
			Initial value   
			&100,000 &100,000&100,000&100,000&100,000&100,000&100,000\\
			Final value     
			&127,044&163,647&174,825&192,031&173,063&172,797&133,402\\
			Annualized return 
			&14.89\%&32.33\% &37.40\%& 44.94\% &36.88\%&36.49\% &17.81\% \\
			Annualized Std &9.63\%&27.51\%&33.41\%&29.62\%&25.84\%&33.41\%&27.00\%\\
			Sharpe ratio      
			& 1.49 & 1.16& 1.12& 1.40& 1.35 & 1.10 &  0.74   \\
			Max drawdown &20.93\%&28.26\%&27.76\%&21.13\%&22.47\%&28.11\%&33.92\%\\
			\hline
		\end{tabular}}
		\caption{Performance of single stock trading using PPO in the FinRL library. The Sharpe ratio of all the ETFs and stocks outperform the market, namely the S\&P 500 index.}
		\label{single_stock_performance}
	\end{table*}
	
	



\begin{table*}[t]
		\centering
		\resizebox{\textwidth}{!}{
		\begin{tabular}{|l|c|c|c|c|c|}\hline
			2019/01/01-2020/09/23 & TD3 & DDPG&  Min-Var. &  DJIA \\
			\hline
			Initial value   
			&1,000,000 &1,000,000&1,000,000&1,000,000\\
			Final value     
			&\textcolor{orange}{1,403,337};~~\textcolor{cyan}{1,381,120}& \textcolor{orange}{1,396,607};~~\textcolor{cyan}{1,281,120}&1,171,120&1,185,260\\
			Annualized return 
			&\textcolor{orange}{21.40\%}; ~~\textcolor{cyan}{17.61\%}&
			\textcolor{orange}{20.34\%}; ~~\textcolor{cyan}{15.81\%}&8.38\%& 10.61\%\\
			Annualized Std 
			&\textcolor{orange}{14.60\%}; ~~\textcolor{cyan}{17.01\%}&
			\textcolor{orange}{15.89\%};~~\textcolor{cyan}{16.60\%}
			&26.21\%&28.63\%\\
			Sharpe ratio      
			& \textcolor{orange}{1.38}; ~~\textcolor{cyan}{1.03}
			&\textcolor{orange}{1.28}; ~~\textcolor{cyan}{0.98} & 0.44 &0.48  \\
			Max drawdown 
			&\textcolor{orange}{11.52\%}~~\textcolor{cyan}{12.78\%}&
			\textcolor{orange}{13.72\%}; ~~\textcolor{cyan}{13.68\%}&34.34\%&37.01\%\\
			\hline
		\end{tabular}}
		\caption{Performance of \textcolor{orange}{multiple stock trading} and \textcolor{cyan}{portfolio allocation} over the DJIA constituents stocks using the FinRL library. The Sharpe ratios of TD3 and DDPG excceed the DJIA index, and the traditional min-variance portfolio allocation strategy.}
		\label{tab:Performance evaluation}
		\vspace{-0.15in}
	\end{table*}
	
\textbf{Risk-aversion}.
Risk-aversion reflects whether an investor will choose to preserve the capital. It also influences one's trading strategy when facing different market volatility level.

To control the risk in a worst-case scenario, such as financial crisis of 2007–2008, FinRL employs the financial turbulence index $\textit{turbulence}_t$ that measures extreme asset price fluctuation \cite{turbulence}:
\begin{equation}  
\textit{turbulence}_t = \left(\bm{y_t} - \bm{\mu}\right)\bm{\Sigma^{-1}}(\bm{y_t}-\bm{\mu})' \in \mathbb{R},
\label{turb}
\end{equation} 
where $\bm{y_t} \in \mathbb{R}^n$ denotes the stock returns for current period t, $\bm{\mu} \in \mathbb{R}^n$ denotes the average of historical returns, and $\bm{\Sigma} \in \mathbb{R}^{n \times n}$ denotes the covariance of historical returns. It is used as a parameter that controls buying or selling action, for example if the turbulence index reaches a pre-defined threshold, the agent will halt buying action and starts selling the holding shares gradually.



\subsection{Demonstration of Three Use Cases}

We demonstrate with three use cases: single stock trading \cite{Dang2019ReinforcementLI,DRL_automate,li_a2c_2018,zhang2020deep}, multiple stock trading \
\cite{xiong2018practical,yang2020}, and portfolio allocation \cite{Jiang2017ADR,li2019optimistic}. FinRL library provides practical and reproducible solutions for each use case, with online walk-through tutorial using Jupyter notebook (e.g., the configurations of the running environment and commands). We select three use cases and reproduce the results using FinRL to establish a benchmark for the quantitative finance community.

Fig. \ref{single_stock} and Table \ref{single_stock_performance} demonstrate the performance evaluation of single stock trading. We pick large-cap ETFs such as SPDR S\&P 500 ETF Trust (SPY) and Invesco QQQ Trust Series 1 (QQQ), and stocks such as Google (GOOGL), Amazon (AMZN), Apple (AAPL), and Microsoft (MSFT). We use PPO algorithm in FinRL and train a trading agent.  The maximum drawdown in Table \ref{single_stock_performance} is large due to Covid-19 market crash.

Fig. \ref{fig3} and Table \ref{tab:Performance evaluation} show the performance and multiple stock trading and portfolio allocation over the Dow Jones 30 constitutes. We use DDPG and TD3 to trade multiple stocks, and allocate portfolio.





==> description/env.tex <==
\section{Environment}

The process of Deep Reinforce Learning is the continuous interaction between agent and environment. Firstly, the agent will receive state(t) from the environment and take action(t) according to its policy. After receiving the action(t) from the agent, the environment will return reward(t+1) and change into state(t+1). Then it would continue the cycle (sequence.png) to maximize the expectation of the rewards. The state(t) includes four properties: price, cash, holding value and holding amount. There are three kinds of actions: buy, sell, hold.
With our library function, the historical data which is stored as common database files will be transformed into environment where the agent could be trained. Then the different algorithms could be called through different functional interface

==> description/frame.tex <==
\section{Framework}

This is the frame of the library function, it mainly depends on Baselines module and Gym module from OpenAI, we build a gym environment based on the financial history data which is a continuous space for deep reinforcement learning's training. Baselines contains algorithms functions and parameter setting functions, then it can support users' direct calls. There are three demos in the project which came from three classic papers in Finance Reinforcement Learning field. In addition,  users can test other Reinforcement Learning algorithms in stock market environment by setting parameters reasonably.

==> old_save/Problem.tex <==

To apply deep reinforcement learning to stock trading, the first step to have an deep reinforcement learning problem formulation, so that the proper definitions of the environment, the agent, states, actions, and rewards functions are very important. 
The process of Deep Reinforce Learning is the continuous interaction between agent and environment. Firstly, the agent will receive state(t) from the environment and take action(t) according to its policy. After receiving the action(t) from the agent, the environment will return reward(t+1) and change into state(t+1). Then it would continue the cycle (sequence.png) to maximize the expectation of the rewards. The state(t) includes four properties: price, cash, holding value and holding amount. There are three kinds of actions: buy, sell, hold. We formulated the stock trading process as a Markov Decision Process (MDP), then it could be solved as a maximization problem through deep reinforcement learning.
In addition, sufficient data are essential for the application of deep reinforcement learning techniques.  With these data, we could build the training environment in gym module, namely feature engineering. This work calls for significant manual effort and financial knowledge. Stock market problems are practical problems, training environments are inevitable and play a vital role in help agent achieving favourable performance.
With environment and problems model, deep reinforcement learning algorithms will be chosen for simulation, rewards function, deep learning network, learning parameters etc. The proposes library functions support to try several algorithms and choose the best one(s), on a case by case basis.
The last step is results' representations, the function output broken line graphs which can effectively help monitor the performance and refine the model accordingly.

\begin{table*}[htb]
\caption{Comparison of DRL Algorithms}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Algorithms}       
& \textbf{Input}        
& \textbf{Output}           
& \textbf{Type}       
& \textbf{State and action space}  
& \textbf{Use cases support}  
& \textbf{Optimization}  
& \textbf{Advantages}  
\\ \hline
\textbf{DQN}       
& States
& Q-value     
& Value Based      
& Discrete only
& Single stock trading
& NN
& Simple
\\ \hline
\textbf{DDPG}       
& State-action pair     
& Q-value     
& Actor-critic based     
& Continuous only 
& Multiple stocks trading, portfolio allocation
& NN
& handle continuous state and action space
\\ \hline
\textbf{PPO}         
& State-action pair      
& Q-value       
& Actor-critic based        
& Discrete and continuous         
& All use cases
& Clipped surrogate objective function
& Improves the stability of the Actor training by limiting the policy update at each training step
\\ \hline
\textbf{A2C}          
& State-action pair      
& Q-value       
& Actor-critic based        
& Discrete and continuous         
& All use cases
& Clipped surrogate objective function
& Improves the stability of the Actor training by limiting the policy update at each training step
\\ \hline
\textbf{SAC}        
& State-action pair      
& Q-value       
& Actor-critic based        
& Discrete and continuous         
& All use cases
& Clipped surrogate objective function
& Improves the stability of the Actor training by limiting the policy update at each training step
\\ \hline
\textbf{TD3}        
& State-action pair      
& Q-value       
& Actor-critic based        
& Discrete and continuous         
& All use cases
& Clipped surrogate objective function
& Improves the stability of the Actor training by limiting the policy update at each training step
\\ \hline
\textbf{Tensorforce}   
& State-action pair      
& Q-value       
& Actor-critic based        
& Discrete and continuous         
& All use cases
& Clipped surrogate objective function
& Improves the stability of the Actor training by limiting the policy update at each training step
\\ \hline
\textbf{Horizon}       
& State-action pair      
& Q-value       
& Actor-critic based        
& Discrete and continuous         
& All use cases
& Clipped surrogate objective function
& Improves the stability of the Actor training by limiting the policy update at each training step
\\ \hline
\end{tabular}
\end{table*}

==> old_save/References.tex <==
\begin{thebibliography}{99}  
%格式不统一
\bibitem{ref1} Hull, J. C. (2014). Options, futures and other derivatives (9th Edition). Prentice Hall.

\bibitem{ref2}Stelios D. Bekiros, Fuzzy adaptive decision-making for boundedly rational traders in speculative stock markets. European Journal of Operational Research, vol. 202, pp. 285-293, 2010.

\bibitem{ref3}Yong Zhang, and Xingyu Yang, Online portfolio selection strategy based on combining experts’ advice. Computational Economics, vol. 50, No. 1, pp. 141-159, 2017.

\bibitem{ref4}Youngmin Kim, Wonbin Ahn, Kyong Joo Oh, and David Enke, An intelligent hybrid trading system for discovering trading rules for the futures market using rough sets and genetic algorithms. Applied Soft Computing, vol. 55, pp. 127-140, 2017.

\bibitem{ref5}Luenberger, D. G. (1997). Investment Science. Oxford University Press.

\bibitem{ref6}Moody, J. and Saffell, M. Learning to trade via direct reinforcement. IEEE Transactions on Neural Networks, 12(4):875–889, 2011.

\bibitem{ref7}Deng, Y., Bao, F., Kong, Y., Ren, Z., and Dai, Q. (2016). Deep direct reinforcement learning for financial signal representation and trading. IEEE Transactions on Neural Networks and Learning Systems.

\bibitem{ref8}Heaton, J. B., Polson, N. G., and Witte, J. H. (2016). Deep learning for finance: deep portfolios. Applied Stochastic Models in Business and Industry.
Heaton, J. B., Polson, N. G., and Witte, J. H. ( 2017) Deep learning for finance: deep portfolios. Appl. Stochastic Models Bus. Ind., 33: 3– 12. 

\bibitem{ref9}Sharpe, W. F. and Sharpe, W. Portfolio theory and capital markets, volume 217. McGraw-Hill New York, 1970.

\bibitem{ref10}Xiong, Z., Liu, X.-Y., Zhong, S., Walid, A., et al. Practical deep reinforcement learning approach for stock trading.NeurlIPS Workshop on Challenges and Opportunities for AI in Financial Services, 2018.
@unknown{unknown,
author = {Xiong, Zhuoran and Liu, Xiao-Yang and Zhong, Shan and Hongyang, and Yang, and Walid, Anwar},
year = {2018},
month = {11},
pages = {},
title = {Practical Deep Reinforcement Learning Approach for Stock Trading}
}
\bibitem{ref11}%adaptive ddpg
Li,X.-Y., Li Y.-C., Zhan Y.-c., and Liu, X.-Y. Optimistic Bull or Pessimistic Bear: Adaptive Deep Reinforcement Learning for Stock Portfolio Allocation. Proceedings of the 36 th International Conference on Machine Learning, Long Beach, California, PMLR 97, 2019.

\bibitem{ref12}
Bao,W.-H., and Liu, X.-Y. Multi-agent reinforcement learning for liquidation strategy analysis. Proceedings of the 36 th International Conference on Machine Learning, Long Beach, California, 2019.

\bibitem{ref13}
Matloff, N. Introduction to discrete-event simulation and the simpy language. Davis, CA. Dept of Computer Science. University of California at Davis. Retrieved on August, 2(2009), pp.1-33.

\bibitem{ref14}
Hao Dong, Akara Supratak, Luo Mai, Fangde Liu, Axel Oehmichen, Simiao Yu, and Yike Guo. 2017. TensorLayer: A Versatile Library for Efficient Deep Learning Development. In Proceedings of the 25th ACM international conference on Multimedia (MM ’17). Association for Computing Machinery, New York, NY, USA, 1201–1204. 

\bibitem{ref15}
Duan, Y. , Chen, X. , Houthooft, R. , Schulman, J. , \& Abbeel, P. . (2016). Benchmarking deep reinforcement learning for continuous control.

\bibitem{ref16}%DDPG
Lillicrap, Timothy P., et al. Continuous control with deep reinforcement learning. arXiv preprint, 2015, 

\bibitem{ref17}
https://github.com/Ceruleanacg/Personae

\bibitem{ref18}
Greg Brockman, Vicki Cheung, Ludwig Pettersson, Jonas Schneider, John Schulman, Jie
Tang, and Wojciech Zaremba. Openai gym. arXiv preprint arXiv:1606.01540, 2016.

\bibitem{ref19}
Silver, D., Huang, A., Maddison, C. et al. Mastering the game of Go with deep neural networks and tree search. Nature 529, 484–489 (2016).

\bibitem{ref20}
Daochen Zha, Kwei-Herng Lai, Yuanpu Cao, Songyi Huang, Ruzhe Wei, Junyu Guo, Xia Hu. arXiv:1910.04376, 2019.

\bibitem{ref21}
Lucian Bu¸soniu, Tim de Bruin, Domagoj Tolic, Jens Kober, Ivana Palunko, “Reinforcement learning for control: Performance, stability, and deep approximators,” Annual Reviews in Control, ISSN 1367-5788, 2018.

\bibitem{ref22}%DQN
"Human-level control through deep reinforcement learning." Nature 518.7540(2015):529-533.

\bibitem{ref23}
Almgren, R. and Chriss, N. Optimal execution of portfolio transactions. Journal of Risk, 3:5–40, 2001.

\bibitem{ref24}
Sharpe, W. F. and Sharpe, W. Portfolio theory and capital markets, volume 217. McGraw-Hill New York, 1970.

\bibitem{ref25}%Q-learning
Ben J. A. Kröse. "Learning from delayed rewards." Robotics and Autonomous Systems 15.4(1995):233-235.

\bibitem{ref26}%maddpg al
Ryan Lowe. Multi-Agent Actor-Critic for Mixed Cooperative-Competitive Environments[J]. 2017.

\bibitem{ref27}
Howard, R.A.．Dynamic Programming and Markov Processes．Cambridge, Massachusetts：Technology Press-Wiley，1960.

\bibitem{ref28}
Brockman, Greg and Cheung, Vicki and Pettersson, Ludwig and Schneider, Jonas and Schulman, John and Tang, Jie and Zaremba, Wojciech. Openai gym. arXiv preprint arXiv:1606.01540, 2016.

\bibitem{ref29}
https://arxiv.org/pdf/1707.06347.pdf

\end{thebibliography}

==> sections/old-RLagents.tex <==
\subsection{Agents: ElegantRL Algorithms}


\begin{figure*}[ht]
\centering
\includegraphics[width=1\textwidth]{image/compare_4.PNG}
\caption{Comparison of DRL Algorithms.}
\label{compare}
\end{figure*}

%\textcolor{red}{Need to add some finance ingredients: continuous state space, high dimension, etc. Refer to the paper on challenges of SOTA DRL.}

%\yanglet{To Bruce, I am looking for a table with descriptions: input, output, loss function, type (like value, policy, actor-critic), optimization skills?  stability, }

The interaction between agent and environment is modeled as a Markov Decision Process (MDP) $\langle \mathcal{S}, \mathcal{A}, \mathcal{T}, r, \gamma \rangle$, where $\mathcal{S}$ denotes the state space, $\mathcal{A}$ denotes the action space, $\mathcal{T}$ denote the transition probability, $r$ denotes the reward function, and $\gamma$ denotes the discount factor. We then specify the input, output and loss function of the DRL agents as well as RL agents. 

%Input is the state $s=[a,h,b]$, reward $r(s,a,s')$. Output: action $a \in \{selling, holding, buying\}$.

% The FinRL library includes both conventional RL and latest DRL agents. The conventional RL algorithms serve as benchmarks for DRL algorithms, which helps debugging and tuning of newly designed DRL agents. 

\subsubsection{Conventional RL Agents} 
Dynamic programming methods are used to maximize the expected return \cite{howard1960dynamic} in MDP, which serves as a benchmark for developing and debugging the deep neural networks.
% assume the stock market satisfies the Markov property, that its future state depends only on the current state. Then one

\textbf{Value Iteration} \cite{howard1960dynamic}: At the current state, the agent estimates the expected value of the next state after taking possible actions 
%and find the action with maximum Q-value:
\begin{equation}
Q_{\pi}(s, a)=\sum_{s^{\prime}} \mathcal{T}\left(s^{\prime} | a, s\right)\left(r\left(s, a, s^{\prime}\right)+\gamma V_{\pi}\left(s^{\prime}\right)\right).
\end{equation}
where $Q_{\pi}(s, a)$ denotes the expected return by following policy $\pi$.
%The maximum expected value function will be the value function of the current state \begin{equation}V_{\pi}(s)=Q_{\pi}(s, \pi(s))\end{equation}


\textbf{Policy Iteration} \cite{bellman1957markovian}: It initializes a random policy $\pi$ at the beginning and estimates the state-value $V(s)$:
\begin{equation}
V(s)=r(s, \pi(s))+\gamma \sum_{s^{\prime}} \mathcal{T}\left(s, \pi(s), s^{\prime}\right) \cdot V\left(s^{\prime}\right).
\end{equation}
Then, update the policy $\pi$ with a greedy strategy:
\begin{equation}
\pi(s) \leftarrow \operatorname{argmax}_{a}\left\{r(s, a)+\gamma \sum_{s^{\prime}} \mathcal{T}\left(s, a, s^{\prime}\right) \cdot V\left(s^{\prime}\right)\right\}.
\end{equation} 
%The optimal policy and the optimal value function are finally obtained through iterations. 
% There are two stages\: (1) Policy evaluation: estimate v(pi) under the given policy. In FinRL, each state has 3 actions {sell, hold and buy}, after each round of estimation, the return of the optional action in the current state is estimated according to the state. (2) Policy improvement: obtain the current policy pi according to the modified policy and the previously obtained v(pi). In FinRL, the action with the highest return is selected to be retained, namely, the probability of the selected action is increased.

\subsubsection{Deep RL Agents}

The FinRL library includes fine-tuned standard DRL algorithms, namely, DQN \cite{lillicrap2015continuous}\cite{mnih2015human}, DDPG \cite{lillicrap2015continuous}, Multi-Agent DDPG \cite{lowe2017multi}, PPO \cite{schulman2017proximal}, SAC \cite{haarnoja2018soft}, A2C \cite{mnih2016asynchronous} and TD3 \cite{Dankwa2019TwinDelayedDA}. We also allow used to design their own DRL algorithms by adapting these DRL algorihtms, e.g, Adaptive DDPG \cite{li2019optimistic}, or by employing ensemble methods.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Deep Q-Network (DQN)}  \cite{lillicrap2015continuous}\cite{mnih2015human}: 
The DQN agent has state $s_{t}$ as input and outputs multiple Q-values $Q(s, a)$ for the allowed actions $a \in \mathcal{A}$. The agent uses a greedy strategy to select the action with the largest $Q(s, a)$. 
The agent updated the network weights by minimizing the loss function \begin{equation}
\begin{array}{l}
L(\theta)=\mathbb{E}\left[(r+\gamma \max _{a^{\prime}} Q\left(s^{\prime}, a \prime ; \theta\right)-Q(s, a ; \theta))^{2}\right]. \\
%\text { Target } Q=r+\gamma \max _{a^{\prime}} Q\left(s^{\prime}, a \prime ; \theta\right)
\end{array}
\end{equation}
% DQN can be used to deal with small amount of stocks' data.% 
FinRL encodes the action space $\mathcal{A} = \{\text{buy}, \text{hold}, \text{sell}\}$ as a discrete set $\{-1, 0, 1\}$ in the DQN algorithm. Since the support action space has limited size, DQN can support stock trading of a small scale.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Deep Deterministic Policy Gradient (DDPG)} \cite{lillicrap2015continuous}: The deep deterministic policy gradient algorithm uses the Actor-Critic framework. The target of DDPG agent is to optimize the policy that maximize $ Q_{\pi}\left(s_{t}, a_{t}\right)$:
\begin{equation}
 \begin{split}
   Q_{\pi}\left(s_{t}, a_{t}\right)=
   &\mathbb{E}_{s_{t+1}}\left[r\left(s_{t}, a_{t}, s_{t+1}\right) +\gamma \mathbb{E}_{a_{t+1} \sim \pi\left(s_{t+1}\right)}\left[Q_{\pi}\left(s_{t+1}, a_{t+1}\right)\right]\right].
 \end{split}
\end{equation}
The loss function over a batch of $N$ transitions $\{s_i, a_i, r_i, s_{i}'\}$ is
\begin{equation}
L=\frac{1}{N} \sum_{i}\left(y_{i}-Q\left(s_{i}, a_{i} | \theta^{Q}\right)\right)^{2},
\label{ddpg_loss}
\end{equation} 
where
$y_i = r_i+\gamma Q' (s_{i}', \mu' (s_{i}' |\theta^{\mu'},\theta^{Q'})), i=1,\cdots,N.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Adaptive Deep Deterministic Policy Gradient} \cite{li2019optimistic}: Different from DDPG, the update of Q-value has been changed to:
\begin{equation}
Q_{\pi}\left(s_{t+1}, a_{t+1}\right)=Q_{\pi}\left(s_{t}, a_{t}\right)+\alpha \delta(t).
\end{equation}
where $\alpha$ is a learning rate, and $\delta(t)$ is the prediction error as follows:
\begin{equation}\delta(t)=r\left(s_{t}, a_{t}, s_{t+1}\right)-Q_{\pi}\left(s_{t}, a_{t}\right).
\end{equation}
The loss function is the same as (\ref{ddpg_loss}).
%\begin{equation}L=\frac{1}{N} \sum_{i}\left(y_{i}-Q\left(s_{i}, a_{i} | \theta^{Q}\right)\right)^{2}\end{equation}
Considering that market information can have a huge impact on the trading agent, Adaptive-DDPG aims to analyze the mechanism of stock information penetration quantitatively.

\textbf{Proximal Policy Optimization (PPO)} \cite{schulman2017proximal}:
%不确定，openai：https://spinningup.openai.com/en/latest/algorithms/ppo.html；原论文：https://arxiv.org/pdf/1707.06347.pdf%
PPO algorithm is a new policy gradient algorithm to deal with the problem that the step size in policy gradient algorithms is difficult to determine. The target function of PPO is updated in small batches:
\begin{equation}\begin{array}{c}
L\left(s, a, \theta_{k}, \theta\right)=\min \left(\frac{\pi_{\theta}(a | s)}{\pi_{\theta_{k}}(a | s)} A^{\pi_{\theta_{k}}}(s, a), g\left(\epsilon, A^{\pi_{\theta_{k}}}(s, a)\right)\right), \\
g(\epsilon, A)=\left\{\begin{array}{cc}
(1+\epsilon) A, & A \geq 0, \\
(1-\epsilon) A, & A<0,
\end{array}\right.
\end{array}\end{equation}
where the advantage function is
$A(s_{t},a_{t}) = Q(s_{t},a_{t}) - V(s_{t})$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Advantage Actor Critic (A2C)} \cite{mnih2016asynchronous}:
A2C is a policy gradient algorithm that adds a baseline to Q-value, and the reward can be positive or negative
The loss function of the critic is
%\begin{equation}L_{\text {critic}} = \frac{1}{N} \sum_{i=0}^{N} \sum_{s, a \in %z_{i}}\left(V_{\theta}(s)-\left[r+\gamma \cdot %V\left(s^{\prime}\right)\right]\right)^{2}
%\end{equation}
\begin{equation}
     L(\theta)=\mathbb{E}\left[\sum_{t=1}^{T}\nabla_{\theta}\log \pi_{\theta}(a_{t}|s_{t})A(s_{t},a_{t}) \right],
\end{equation}
where $\pi_{\theta}(a_{t}|s_{t})$ is the policy network.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Soft Actor-Critic (SAC)} \cite{haarnoja2018soft}: %https://spinningup.openai.com/en/latest/algorithms/sac.html%
SAC is an off-policy, maximum entropy, actor-critic algorithm. The loss function is
\begin{equation}L\left(\phi_{i}, \mathcal{D}\right)=\underset{\left(s, a, r, s^{\prime}, d\right) \sim \mathcal{D}}{\mathrm{\mathbb{E}}}\left[\left(Q_{\phi_{i}}(s, a)-y\left(r, s^{\prime}, d\right)\right)^{2}\right]\end{equation}
and the target function is
\begin{equation}
\begin{split}
y\left(r, s^{\prime}, d\right) =&r+\gamma(1-d)\left(\min _{j=1,2} Q_{\phi_{\mathrm{\text{targ}}, j}}\left(s^{\prime}, \tilde{a}^{\prime}\right)-\alpha \log \pi_{\theta}\left(\tilde{a}^{\prime} | s^{\prime}\right)\right), \\
&\tilde{a}^{\prime} \sim \pi_{\theta}\left(\cdot | s^{\prime}\right).
\end{split}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Twin Delayed DDPG (TD3)} \cite{fujimoto2018addressing}:
TD3 uses two Q-nets to optimize the overestimation problem of Q-value in DDPG. These two Q-nets share the same target:
\begin{equation}
y\left(r, s^{\prime}, d\right)=r+\gamma(1-d) \min _{i=1,2} Q_{\phi_{i, \text { targ }}}\left(s^{\prime}, a^{\prime}\left(s^{\prime}\right)\right).
\end{equation}
Then they are learned through the smaller one of the two loss functions:
\begin{equation}
\begin{array}{l}
L\left(\phi_{1}, \mathcal{D}\right)=\underset{\left(s, a, r, s^{\prime}, d\right) \sim \mathcal{D}}{\mathrm{\mathbb{E}}}\left[\left(Q_{\phi_{1}}(s, a)-y\left(r, s^{\prime}, d\right)\right)^{2}\right], \\
L\left(\phi_{2}, \mathcal{D}\right)=\underset{\left(s, a, r, s^{\prime}, d\right) \sim \mathcal{D}}{\mathrm{\mathbb{E}}}\left[\left(Q_{\phi_{2}}(s, a)-y\left(r, s^{\prime}, d\right)\right)^{2}\right].
\end{array}
\end{equation}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Multi-Agent Deep Deterministic Policy Gradient} \cite{bao2019multi}: Most of the successes of RL algorithms have been in a single agent case, where modelling or predicting the behaviors of other actors is not considered. The obtained trading strategy ignores the stochastic and interactive nature of the trading market. A more general scenario would be that multiple organizations or customers want to conduct trading actions at the same time. Multi-agent DDPG assumes $J$ agents, each agent has $X_{j}$ shares to sell within a given time frame $T$. Then the target is making the total expected shortfall larger than or equal to the sum of expected shortfalls in a single-agent environment:
\begin{equation}
\sum_{j=1}^{J} \mathbb{E}\left(X_{j}\right) \leq \mathbb{E}\left(\sum_{j=1}^{J} X_{j}\right).
\end{equation}
The loss function is $L=$ $\frac{1}{N} \sum_{i}\left(y_{j, i}-Q_{j}\left(O_{j, i}, a_{j, i} | \theta_{j}^{Q}\right)\right)^{2}$. 


%所有期望符号 统一 \mathbb{E}

\subsection{SOTA Performance}
